Automated Implementation of Windows-related Security-Configuration Guides

Hardening is the process of configuring IT systems to ensure the security of the systems' components and data they process or store. The complexity of contemporary IT infrastructures, however, renders manual security hardening and maintenance a daunting task. In many organizations, security-configuration guides expressed in the SCAP (Security Content Automation Protocol) are used as a basis for hardening, but these guides by themselves provide no means for automatically implementing the required configurations. In this paper, we propose an approach to automatically extract the relevant information from publicly available security-configuration guides for Windows operating systems using natural language processing. In a second step, the extracted information is verified using the information of available settings stored in the Windows Administrative Template files, in which the majority of Windows configuration settings is defined. We show that our implementation of this approach can extract and implement 83% of the rules without any manual effort and 96% with minimal manual effort. Furthermore, we conduct a study with 12 state-of-the-art guides consisting of 2014 rules with automatic checks and show that our tooling can implement at least 97% of them correctly. We have thus significantly reduced the effort of securing systems based on existing security-configuration guides.

==> contents/03_overview.tex <==
\section{Windows-related Security Configuration: Generic Approach}
\label{sec:genericapproach}

\begin{figure*}
    \includegraphics[width=\textwidth]{images/approach.pdf}
    \caption{Overview of the abstract hardening approach.}
    \label{fig:hardeningAppraoch}
\end{figure*}

In this section, we introduce a generic approach for automatically implementing Windows-related security-configuration guides.
Figure~\ref{fig:hardeningAppraoch} shows the different stages of the envisioned process.
This generic approach is the foundation for our actual approach which is explained in the following section.

We see the security-configuration guides as the natural input to an automated security configuration process.
In a first step, the \textit{Extraction}, we need to extract all the information necessary to implement to guide.
In the current process, an administrator has to do this manually by going through the guide and find for each rule this information;
in an automated approach, this has to be done automatically.
The next step, the \textit{Verification}, we verify that the given settings exist and values are valid for that setting.
This step is especially important for internal guides because it reduces the amount of configuration errors resulting from typing errors etc.
Currently, the administrators has to look up if the setting exists and then compare the given value with the possible values.
In the third step, the \textit{Transformation to low-level}, we translate the high-level description in the rule into an executable form.
For most of the settings, the administrators has to look up which registry is changed by the given settings and how the values are translated.
In the fourth step, the \textit{Transformation to code}, we create executable code from the output of Step~3.
Our idea here is that the output of Step~4 contains all the information we need to automatically implement the rules;
thus, we only need to ship the output of Step~4 to the system under test.
Nowadays, the administrator creates with the information of Step~3 PowerShell scripts or something similar to implement the rules.
The last step we envision is the actual \textit{Implementation}.
This is the only step which we have to execute on the system under test.
We can also execute the other steps on the system under test, but we do not have to.
In this step, we implement the rules by executing the output of Step~4.
The result of this generic approach is a system under test which is configured as specified in the guide.
If the complete implementation of the guide leads to a secure system, the system under test will be secure.

==> contents/04_overview.tex <==
\section{Overview}
\label{sec:overview}

After we introduced the generic approach, we present in this section the approach we have implemented following the general ideas.
Before we talk about the technical details of the Windows-related security configuration, we first explain the steps in an abstract way.

Our abstract approach is aligned with the phases of Figure~\ref{fig:hardeningAppraoch} and consists of the following steps.

\begin{itemize}
    \item[\textbf{Extraction:}] Use natural-language processing for each rule to extract the information needed to implement this rule automatically
    \item[\textbf{Verification:}] Devise an automated mechanism that checks whether the derived information is valid:
    \begin{itemize}
        \item Does the extracted policy path indeed exist?
        \item Has the extracted value the required type for that setting?
        \item Does the extracted value meet the requirements of that setting?
        Is it in the list of possible values or in the range of allowed values?
    \end{itemize}
    if the path or the value are incorrect, the mechanism provides useful feedback about possible paths or values.
    \item[\textbf{Transformation to low-level:}] Transform GPO settings into a representation of one of the underlying \textit{low-level} implementation mechanisms.
    This step is necessary because almost none of the most popular configuration-management frameworks can directly process GPO settings, but require the specification of an underlying implementation mechanism:
    \begin{itemize}
        \item Registry settings
        \item Secedit policy file entries
        \item Audit file entries.
    \end{itemize}
    \item[\textbf{Transformation to code:}] Transform these low-level implementation mechanisms into code for carrying out the implementation of each setting.
    \item[\textbf{Implementation:}] Execute code on the system to be hardened to implement the rules
\end{itemize}

After discussing the abstract steps of our approach, we proceed with the technical details of our implementation.

